Towards Evaluation Engineering: An Empirical Study of ML Evaluation Harnesses in the Wild

Evaluation harnesses are software systems that orchestrate model evaluation by managing model invocation, data loading, metric computation, and result reporting. Despite their critical role in machine learning infrastructure, their operational challenges and engineering concerns have received limited attention so far. We present an empirical study of 57 evaluation harnesses, deriving a five-stage harness model and classifying 16,560 issues by workflow stage and root cause. Most harness operational challenges concentrate in the Specification stage (41.4% of issues), where harnesses integrate external models, datasets, and scoring judges. The three most frequent root causes of operational challenges are unimplemented features (24.3%), documentation gaps (20.3%), and missing input validation (17.2%), which together account for 61.7% of classified issues, spanning both defects in existing functionality and capability gaps that block intended workflows. Root causes also vary by workflow stage: environment incompatibility and external dependency breakage account for 36.2% of provisioning issues, whereas algorithmic error (25.9%) and validation gap (22.5%) dominate assessment issues. Together, these contributions establish an empirical foundation for treating evaluation engineering as a distinct software engineering concern.

==> sections/authors-bio.tex <==
\begin{IEEEbiography}    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/ZhiminZhao.jpg}}]{Zhimin Zhao} is currently pursuing a PhD degree in the Software Analysis and Intelligence Lab (SAIL), Queen's University, Canada. He received his MSE degree from the SIG Center for Computer Graphics at the University of Pennsylvania, USA. He has served as a program committee member for MSR. His research interests include LLMOps, MLOps, and SE4AI. For more details on his work, visit https://zhimin-z.github.io.
\end{IEEEbiography}

\begin{IEEEbiography}    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/ZehaoWang.jpg}}]{Zehao Wang} is a Ph.D. student in the Department of Computer Science and Software Engineering at Concordia University, Montreal, Canada. His research interests include software performance, LLM agents, distributed systems, and AI4SE. His work has been published in conferences, such as ICSE, FSE, and JSS. He served as a program committee member for MSR. He obtained his B.Sc. from Xidian University and M.Sc. from Concordia University. More information at: https://zehaowang00.github.io/
\end{IEEEbiography}

\begin{IEEEbiography}    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/AbdulAliBangash.jpg}}]{Abdul Ali Bangash} is an Assistant Professor at the Lahore University of Management Sciences (LUMS), Pakistan, where he leads the Software Engineering for Good (SFG) research group. He completed his PhD in Computer Science from the University of Alberta, Canada, in 2023. His research lies at the intersection of software engineering and artificial intelligence, including software engineering for AI systems and the application of AI techniques to software engineering. His work has been published in leading software engineering venues such as ICSE, MSR, ICSME, TSE, and EMSE. He has also served as a reviewer and program committee member for top-tier venues including TSE, TOSEM, ICSE, MSR, and ICSME. For more details on his work, visit: http://abdulali.github.io
\end{IEEEbiography}

\begin{IEEEbiography}    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/BramAdams.jpg}}]{Bram Adams} is a full professor at Queen's University (up to June 2020: Polytechnique Montreal). He obtained his PhD in 2008 at Ghent University's GH-SEL laboratory (Belgium). His research interests include software release engineering, software engineering for artificial intelligence (AI) (and vice versa), and mining software repositories. His work received the Foundational Contribution Award for 2021 Mining Software Repositories. In addition to co-organizing the RELENG International Workshop on Release Engineering from 2013 to 2015 (and the 1st/2nd IEEE Software Special Issue on Release Engineering), he co-organized, amongst others, SEMLA 2018/19, FM+SE Vision 2030, and AIware 2024. He has been PC co-chair of SCAM 2013, SANER 2015, ICSME 2016, and MSR 2019; software analytics area co-chair of ICSE 2023, and general chair of MSR 2025. He is a Senior IEEE Member.
\end{IEEEbiography}

\begin{IEEEbiography}    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author/AhmedEHassan.jpg}}]{Ahmed E. Hassan} is an ACM Fellow, IEEE Fellow, and NSERC Steacie Fellow. He is a laureate of the Mustafa Prize, a distinction equivalent in prestige to a Nobel, for founding the AI-augmented SE field and its associated Mining Software Repositories (MSR) conference. He is a Distinguished Educator of IEEE TCSE and an Influential Educator of ACM SIGSOFT. He is a recipient of the inaugural New Directions IEEE TCSE Award for his outstanding and sustained efforts to advance the field of AI-augmented SE. He is the Canada Research Chair (CRC) in Software Analytics and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen's University, Canada. For more details on his work, visit http://sail.cs.queensu.ca.
\end{IEEEbiography}
